Analytical and numerical study of a modified cell problem for the numerical homogenization of multiscale random fields

A central question in numerical homogenization of partial differential equations with multiscale coefficients is the accurate computation of effective quantities, such as the homogenized coefficients. Computing homogenized coefficients requires solving local corrector problems followed by upscaling relevant local data. The most naive way of computing homogenized coefficients is by solving a local elliptic problem, which is known to suffer from the so-called resonance error dominating all other errors inherent in multiscale computations. A far more efficient modelling strategy, based on adding an exponential correction term to the standard local elliptic problem, has recently been proved to result in exponentially decaying error bounds with respect to the size of the local geometry. The questions in relation with the accuracy and computational efficiency of this approach has been previously addressed in the context of periodic homogenization. The present article concerns the extension of mathematical and numerical study of this modified elliptic corrector problem to stochastic homogenization problems. In particular, we assume a stationary, ergodic micro-structure and i) establish the well-posedness of the corrector equation, ii) analyse the bias (or the systematic error) originating from additional exponential correction term in the model. Numerical results corroborating our theoretical findings are presented.

==> tex/naive_approach.tex <==
The most natural approach for approximating the homogenized coefficient is to replace the infinite domain formulations \eqref{eq: ell corr spat prob}-\eqref{eq: a0} by 
\begin{equation}\label{eq: ell corr spat prob domain R}
\left\lbrace
\begin{aligned}
-\nabla\cdot\left(a(x)\left(\nabla\chi_R + \xi\right)\right) &= 0 &\quad&\text{ in }K_R:=(-R/2,R/2)^d, \\
\chi_R &= 0 & \quad & \text{on } \partial K_R ,
\end{aligned}
\right.
\end{equation}
and 
\begin{equation}
\label{eq: a0RL}
\xi \cdot a^{0,R,L}\xi = \fint_{K_L} \left(\nabla \chi_R + \xi\right) \cdot a(x) \left(\nabla \chi_R + \xi\right) \,dx,
\end{equation}
with  $K_L:=(-L/2,L/2)^d\subset K_R$. In theory any $1\leq L \le R$ may be chosen in \eqref{eq: a0RL}, but for computational efficiency, $L = \mathcal{O}(R)$ is preferred in practice. We implicitly assume that $L=\mathcal{O}(R)$ although we keep the notation $L$ as a separate parameter to indicate that the size of the averaging domain $|K_L|$ may be different than $|K_{R}|$. Note that the Dirichlet boundary conditions (BCs) in \eqref{eq: ell corr spat prob domain R}, may be safely replaced by other BCs, e.g. periodic or homogeneous Neumann BCs. 
The approximation error between $a^{0,R,L}$ and $a^{0}$ is measured in a mean square sense as 
\begin{equation} \label{Ineq:Error_Split1}
%\begin{split}
\sup\limits_{\xi\in\R^d,\norm{\xi}=1}\E{\abs{\xi \cdot (a^{0,R,L}- a^0)\xi}) ^2}^{\frac{1}{2}}
\le \underbrace{\sup\limits_{\xi\in\R^d,\norm{\xi}=1}\E{\abs{\xi \cdot (a^{0,R,L}- a^{0,L})\xi} ^2}^{\frac{1}{2}} 
}_{\text{boundary error}}
%&+ \underbrace{\sup\limits_{\xi\in\R^d,\norm{\xi}=1}\E{\abs{\xi \cdot (a^{0,L}- a^{0})\xi} ^2}^{\frac{1}{2}}
%}_{\text{statistical error}} .
+ \underbrace{\sup\limits_{\xi\in\R^d,\norm{\xi}=1}\sqrt{\var{\xi \cdot a^{0,L}\xi}} 
}_{\text{statistical error}} .
%\end{split}
\end{equation}
%The mean square error between $a^{0,R,L}$ and $a^{0}$ can then be split into two terms as follows
%\begin{equation} \label{Ineq:Error_Split1}
%\E{\abs{\xi \cdot (a^{0,R,L}- a^0)\xi}) ^2}^{\frac{1}{2}}
%\le
%\E{\abs{\xi \cdot (a^{0,R,L}- a^{0,L})\xi} ^2}^{\frac{1}{2}} 
%+ \E{\abs{\xi \cdot (a^{0,L}- a^{0})\xi} ^2}^{\frac{1}{2}} .
%\end{equation}
Here, the term $a^{0,L}$ is a random variable approximating the homogenized coefficient, i.e. ${\E{a^{0,L}}=a^0}$, and it is computed by replacing $\chi_{R}$ in formula \eqref{eq: a0RL} by the solution $\chi$ to \eqref{eq: ell corr spat prob}. The first term in the right-hand side of \eqref{Ineq:Error_Split1} is due to the mismatch between the values of $\chi$ and $\chi_R$ on the boundary $\partial K_{R}$, while the second term accounts for the \emph{statistical} error, due to the averaging of a finite number of samples. The boundary error is known to be $\mathcal{O}(R^{-\alpha})$ with $0<\alpha\leq 1$, \cite{BoP04,Yur86}. The convergence rate is known to be of first order ($\alpha=1$) for periodic coefficients, while it is typically worse in the random case. In dimension $d=1$ the convergence rate is proven to be $\alpha=1/2$, while $\alpha\approx\frac{6}{25}$ in dimension $d=3$, \cite{EMZ05}. On the other hand, the statistical error scales as $\mathcal{O}(L^{-d/2})$, which is the optimal rate due to the central limit theorem. Therefore the boundary error dominates the  errors due to discretization and statistical averaging, which is also present in typical multiscale numerical methods, and better strategies are needed to bring this error down to practical tolerances of interests. 

Several interesting approaches have recently been proposed to reduce the above mentioned boundary error, see \cite{AAP19a,AAP19c,AAP19b,ArR16b,BlL10,CEL15b,Glo08,GlH16,HMS19}, where the core idea relies on modifying the corrector problem \eqref{eq: ell corr spat prob domain R} so that the artificial boundary conditions imposed on the boundary $\partial K_{R}$ has a minor influence on the accuracy of the approximate homogenized coefficient. In the remaining part of the introduction, we briefly mention two successful approaches from \cite{AAP19c,Glo08}, which use elliptic corrector problems.

==> tex/numerical_experiments.tex <==
In this section we collect the results of numerical experiments performed in order to:
\begin{itemize}
	\item verify numerically the exponential convergence of the boundary error in the context of random coefficients;
	\item verify numerically the correctness of the proved bound on the systematic error in Theorem \ref{thm: systematic error};
	\item compare the convergence of the global modelling error for the standard numerical homogenization scheme and for the modified elliptic approach.
\end{itemize}
The convergence of the error is measured with respect to the modelling parameters $R$, $L$ and $T$. 
As we already saw in \Cref{sec: intro}, the mean square error can be bounded by the sum of three terms: the boundary, the systematic and the statistical errors.
In order to avoid that the approximation error is dominated by the statistical error (which is often the case when $L$ is not chosen large enough), we looked at the error in mean, i.e.,
\begin{equation}\label{eq:mean err}
e_{M} := \sup\limits_{\xi\in\R^d,\norm{\xi}=1} \abs{  \xi \cdot \E{a^{0,R,L,T}- a^0}\xi  }.
\end{equation}
The advantage of using this error measure is that it does not depend on the statistical error, allowing for experimentally testing the decay of the sum of boundary and systematic errors. This is clear from the decomposition: 
\begin{equation*}
\abs{ \xi \cdot \E{a^{0,R,L,T}- a^0}\xi } 
\le 
\abs{ \xi \cdot \E{a^{0,R,L,T}- a^{0,L,T}}\xi } 
+ \underbrace{ \abs{ \xi \cdot \E{a^{0,L,T}- a^{0,T}}\xi } }_{=0\text{, by \eqref{eq: identity a0T} } }
+ \abs{ \xi \cdot \E{a^{0,T}- a^0}\xi },
\end{equation*}
thus implying that 
\begin{equation*}
e_{M} \le \underbrace{  \sup\limits_{\xi\in\R^d,\norm{\xi}=1} \abs{ \xi \cdot \E{a^{0,R,L,T}- a^{0,L,T}}\xi } }_{\text{boundary error} }
+ \underbrace{  \sup\limits_{\xi\in\R^d,\norm{\xi}=1} \abs{ \xi \cdot \left(a^{0,T}- a^{0}\right)\xi } }_{\text{systematic error} }.
\end{equation*}
The boundary error has a deterministic upper bound that converges exponentially with exponent $\frac{-\abs{R-L}^2}{T}$, see \Cref{Table_Comparison_Error_Estimates}, while the systematic error decays as $T^{-d/2}$, as proved in \Cref{sec:main results}. Computing $e_M$ \emph{exactly} is not possible, because it relies on an integral formulation over the probability space $\Omega$, but we approximate it by computing the empirical average
\begin{equation}
\label{eq: empirical average}
\bar{a}^{0,R,L,T,N} = \frac{1}{N} \sum_{k=1}^{N} a^{0,R,L,T,k},
\end{equation}
converging to $\E{a^{0,R,L,T}}$ in probability, by the weak law of large numbers. Upon choosing a sufficiently large number of samples, $N$, the difference between $\bar{a}^{0,R,L,T,N} $ and $\E{a^{0,R,L,T}} $ can be made negligible. 
%
%\subsection{One dimensional random checker board}
%Here we describe the results of numerical experiments run with a one dimensional random checker board coefficients \textcolor{red}{[TO BE DELETED]}
%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/RandomCheckerBoard1D/bias"}
%	\end{subfigure}	
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/RandomCheckerBoard1D/std"}
%	\end{subfigure}	
%	\caption{One dimensional random checker board. 
%		Comparison of the error in mean and the mean square error in the standard and modified elliptic models, for a micro domain of increasing size $R$. 
%		We sampled $N=1000$ realizations of the stochastic environment.}
%	\label{fig:bias_std}
%\end{figure}
%
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/RandomCheckerBoard1D/bias_RLfixed"}
%	\end{subfigure}	
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/RandomCheckerBoard1D/std_RLfixed"}
%	\end{subfigure}	
%	\caption{One dimensional random checker board. 
%		Comparison of the bias and statistical error in the standard and modified elliptic models, for a micro model of fixed parameters $R=100, L=50$. 
%		The parameter $k_T$ was chosen very small ($k_T=10^{-3}$) in order to increase the effect of the bias error over the boundary error.
%		We sampled $N=1000$ realizations of the stochastic environment.}
%\end{figure}
%
%\subsection{Two dimensional random checker board}
%Here we describe the results of numerical experiments run with a two dimensional random checker board coefficients \textcolor{red}{[TO BE DELETED]}
%
%\begin{figure}[b!]
%	\centering
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/RandomCheckerBoard2D/bias"}
%	\end{subfigure}	
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/RandomCheckerBoard2D/std"}
%	\end{subfigure}	
%	\caption{Two dimensional random checker board. 
%		Convergence of the bias and statistical errors with respect to $R$, for modelling parameters $T,L = \mathcal{O}(R)$. 
%		We sampled $N=200$ realizations of the stochastic environment.}
%	\label{fig:bias_std 2D}
%\end{figure}
%
%%\begin{figure}[h!]
%%	\centering
%%	\begin{subfigure}{.45\textwidth}
%%		\input{"../img/RandomCheckerBoard2D/bias_RLfixed"}
%%	\end{subfigure}	
%%	\begin{subfigure}{.45\textwidth}
%%		\input{"../img/RandomCheckerBoard2D/std_RLfixed"}
%%	\end{subfigure}	
%%	\caption{Two dimensional random checker board. 
%%		Convergence of the bias and statistical errors with respect to $T$, for ``large enough'' parameters $R=30,L = 15$.		
%%		We sampled $N=500$ realizations of the stochastic environment.}
%%	\label{fig:bias_std 2D RL fixed}
%\end{figure}
